Unaligned Image-to-Image Translation by Learning to Reweight

Unsupervised image-to-image translation aims at learning the mapping from the source to target domain without using paired images for training. An essential yet restrictive assumption for unsupervised image translation is that the two domains are aligned, e.g., for the selfie2anime task, the anime (selfie) domain must contain only anime (selfie) face images that can be translated to some images in the other domain. Collecting aligned domains can be laborious and needs lots of attention. In this paper, we consider the task of image translation between two unaligned domains, which may arise for various possible reasons. To solve this problem, we propose to select images based on importance reweighting and develop a method to learn the weights and perform translation simultaneously and automatically. We compare the proposed method with state-of-the-art image translation approaches and present qualitative and quantitative results on different tasks with unaligned domains. Extensive empirical evidence demonstrates the usefulness of the proposed problem formulation and the superiority of our method.

==> tmp.tex <==
\begin{figure*}[ht]
\begin{subfigure}{.23\textwidth}
  \centering
  % include first image
  \includegraphics[width=.8\linewidth]{latex/figures/supp/assumptions/loss_trend/lineplot_hs2zd_global.png}  
  \caption{$H_S\rightarrow Z_D$-local}
  \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
  \centering
  % include second image
  \includegraphics[width=.8\linewidth]{latex/figures/supp/assumptions/loss_trend/lineplot_hs2zd_local.png}  
  \caption{$Z_D\rightarrow H_S$-global}
  \label{fig:sub-second}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
  \centering
  % include first image
  \includegraphics[width=.8\linewidth]{latex/figures/supp/assumptions/loss_trend/lineplot_zd2hs_global.png}  
  \caption{$Z_D\rightarrow H_S$-local}
  \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
  \centering
  % include second image
  \includegraphics[width=.8\linewidth]{latex/figures/supp/assumptions/loss_trend/lineplot_zd2hs_local.png}  
  \caption{$Z_D\rightarrow H_S$-global}
  \label{fig:sub-second}
\end{subfigure}
\caption{The trend for the term $(1-D_Y(G(x)))^2$ ($(1-D_X(F(x)))^2$) with the global discriminator and the local discriminator for the task $H_S\leftrightarrow Z_d$.}
\label{fig:trend_hs2zd}
\end{figure*}

\begin{figure*}[ht]
\begin{subfigure}{.23\textwidth}
  \centering
  % include first image
  \includegraphics[width=.8\linewidth]{latex/figures/supp/assumptions/loss_trend/lineplot_ch2da_global.png}  
  \caption{$C_H\rightarrow D_A$-local}
  \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
  \centering
  % include second image
  \includegraphics[width=.8\linewidth]{latex/figures/supp/assumptions/loss_trend/lineplot_ch2da_local.png}  
  \caption{$C_H\rightarrow D_A$-global}
  \label{fig:sub-second}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
  \centering
  % include first image
  \includegraphics[width=.8\linewidth]{latex/figures/supp/assumptions/loss_trend/lineplot_da2ch_global.png}  
  \caption{$D_A\rightarrow C_H$-local}
  \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
  \centering
  % include second image
  \includegraphics[width=.8\linewidth]{latex/figures/supp/assumptions/loss_trend/lineplot_da2ch_local.png}  
  \caption{$D_A\rightarrow C_H$-global}
  \label{fig:sub-second}
\end{subfigure}
\caption{The trend for the term $(1-D_Y(G(x)))^2$ ($(1-D_X(F(x)))^2$) with the global discriminator and the local discriminator for the task $C_H\leftrightarrow D_A$.}
\label{fig:trend_ch2da}
\end{figure*}

\begin{figure*}[ht]
\begin{subfigure}{.23\textwidth}
  \centering
  % include first image
  \includegraphics[width=.8\linewidth]{latex/figures/supp/assumptions/loss_trend/lineplot_tb2le_global.png}  
  \caption{$H_S\rightarrow Z_D$-local}
  \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
  \centering
  % include second image
  \includegraphics[width=.8\linewidth]{latex/figures/supp/assumptions/loss_trend/lineplot_tb2le_local.png}  
  \caption{$Z_D\rightarrow H_S$-global}
  \label{fig:sub-second}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
  \centering
  % include first image
  \includegraphics[width=.8\linewidth]{latex/figures/supp/assumptions/loss_trend/lineplot_le2tb_global.png}  
  \caption{$Z_D\rightarrow H_S$-local}
  \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
  \centering
  % include second image
  \includegraphics[width=.8\linewidth]{latex/figures/supp/assumptions/loss_trend/lineplot_le2tb_local.png}  
  \caption{$Z_D\rightarrow H_S$-global}
  \label{fig:sub-second}
\end{subfigure}
\caption{The trend for the term $(1-D_Y(G(x)))^2$ ($(1-D_X(F(x)))^2$) with the global discriminator and the local discriminator for the task $H_S\leftrightarrow Z_d$.}
\label{fig:trend_le2tb}
\end{figure*}


\begin{figure*}
\begin{subfigure}{.48\textwidth}
    

    \centering
    \begin{tabular}{ccccc}
    Input  & 30&50&100&200\\ 
         \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/1_0.jpg}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/1_30.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/1_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/1_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/1_200.png}} \\
             
                     \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/2_0.jpg}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/2_30.png}} & 
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/2_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/2_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/2_200.png}} \\
              \vspace{0.3 cm}
                     \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/3_0.jpg}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/3_30.png}} &
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/3_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/3_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/3_200.png}} \\
             
             %\hdashline
             %\cdashline{1-10}
             
               \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/4_0.jpg}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/4_30.png}} &
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/4_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/4_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/4_200.png}} \\
             
               \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/5_0.jpg}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/5_30.png}} &
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/5_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/5_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/5_200.png}} \\
             
              \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/6_0.jpg}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/6_30.png}} &
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/6_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/6_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/lion2tiger/6_200.png}} 
    \end{tabular}
    \caption{Comparison on the translation $L_E\rightarrow T_B$}.
    \label{fig:my_label}
\end{subfigure}
\hfill
\begin{subfigure}{.48\textwidth}
    \centering
    \begin{tabular}{ccccc}
    Input  & 30&50&100&200\\ 
      \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/4_0.jpg}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/4_30.png}} &
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/4_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/4_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/4_200.png}} \\
             
               \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/5_0.jpg}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/5_30.png}} &
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/5_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/5_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/5_200.png}} \\
             \hdashline
             \vspace{0.3 cm}
                           \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/6_0.jpg}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/6_30.png}} &
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/6_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/6_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/6_200.png}} \\ 
             
         \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/1_0.jpg}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/1_30.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/1_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/1_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/1_200.png}} \\
             
                     \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/2_0.jpg}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/2_30.png}} & 
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/2_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/2_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/2_200.png}} \\
              
                     \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/3_0.jpg}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/3_30.png}} &
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/3_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/3_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/tiger2lion/3_200.png}} 
             
             
             
    \end{tabular}
    \caption{Comparison on the translation $T_B\rightarrow L_E$}.
    \end{subfigure}
    \caption{Comparison on the translation $L_E\leftrightarrow T_B$}.
    \label{fig:my_label}
\end{figure*}


\begin{figure*}
\begin{subfigure}{.48\textwidth}
    

    \centering
    \begin{tabular}{ccccc}
    Input  & 30&50&100&200\\ 
         \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/1_0.png}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/1_30.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/1_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/1_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/1_200.png}} \\
             
                     \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/2_0.png}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/2_30.png}} & 
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/2_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/2_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/2_200.png}} \\
              \vspace{0.3 cm}
                     \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/3_0.png}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/3_30.png}} &
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/3_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/3_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/3_200.png}} \\
             
           
             %\hdashline
             %\cdashline{1-10}
             
               \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/4_0.png}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/4_30.png}} &
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/4_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/4_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/4_200.png}} \\
             
               \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/5_0.png}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/5_30.png}} &
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/5_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/5_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/5_200.png}} \\
             
              \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/6_0.png}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/6_30.png}} &
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/6_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/6_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/zebra2horse/6_200.png}} 
    \end{tabular}
    \caption{Comparison on the translation $Z_D\rightarrow H_S$}.
    \label{fig:my_label}
\end{subfigure}
\hfill
\begin{subfigure}{.48\textwidth}
    \centering
    \begin{tabular}{ccccc}
    Input  & 30&50&100&200\\ 
      %\frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/1_0.png}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/1_30.png}} &  
       %      \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/1_50.png}} &  
    %         \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/1_100.png}} &  
    %         \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/1_200.png}} \\
             
                     \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/2_0.png}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/2_30.png}} & 
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/2_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/2_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/2_200.png}} \\
              \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/7_0.png}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/7_30.png}} & 
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/7_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/7_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/7_200.png}} \\
              \vspace{0.3 cm}
              
                     \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/3_0.png}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/3_30.png}} &
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/3_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/3_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/3_200.png}} \\
             
      \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/4_0.png}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/4_30.png}} &
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/4_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/4_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/4_200.png}} \\
             
               \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/5_0.png}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/5_30.png}} &
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/5_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/5_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/5_200.png}} \\
             \hdashline
             
                           \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/6_0.png}}&  \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/6_30.png}} &
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/6_50.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/6_100.png}} &  
             \frame{\includegraphics[width=1.6cm,height=1.6cm]{latex/figures/supp/assumptions/horse2zebra/6_200.png}} 
             
       
             
             
             
    \end{tabular}
    \caption{Comparison on the translation $H_S\rightarrow Z_D$}.
    \end{subfigure}
    \caption{Comparison on the translation $H_S\leftrightarrow Z_D$}.
    \label{fig:my_label}
\end{figure*}
